Breaking with Fixed Set Pathology Recognition through Report-Guided Contrastive Training

When reading images, radiologists generate text reports describing the findings therein. Current state-of-the-art computer-aided diagnosis tools utilize a fixed set of predefined categories automatically extracted from these medical reports for training. This form of supervision limits the potential usage of models as they are unable to pick up on anomalies outside of their predefined set, thus, making it a necessity to retrain the classifier with additional data when faced with novel classes. In contrast, we investigate direct text supervision to break away from this closed set assumption. By doing so, we avoid noisy label extraction via text classifiers and incorporate more contextual information. We employ a contrastive global-local dual-encoder architecture to learn concepts directly from unstructured medical reports while maintaining its ability to perform free form classification. We investigate relevant properties of open set recognition for radiological data and propose a method to employ currently weakly annotated data into training. We evaluate our approach on the large-scale chest X-Ray datasets MIMIC-CXR, CheXpert, and ChestX-Ray14 for disease classification. We show that despite using unstructured medical report supervision, we perform on par with direct label supervision through a sophisticated inference setting.

==> figures/ablations_head.tex <==
\begin{figure}
    \centering
    \begin{tabular}{ccc}
       \includegraphics[width=0.3\linewidth]{example-image-a}  & \includegraphics[width=0.3\linewidth]{example-image-b} & \includegraphics[width=0.3\linewidth]{example-image-c} \\
    \end{tabular}
    \caption{Performance differences based on chosen output head. On the left the baseline prompts impact on the different heads, in the center the impact of the proposed prompt structures on the best method, on the right the impact of additional data.}
    \label{fig:head}
\end{figure}

==> figures/embeddings.tex <==
\begin{figure}
    \centering
    \begin{tabular}{cccc}
    \toprule
        Supervised & SIMCLR & CLIP & ours  \\
        \midrule
        \includegraphics[width=0.225\linewidth, height=0.225\linewidth]{example-image-a} &
        \includegraphics[width=0.225\linewidth, height=0.225\linewidth]{example-image-a} & 
        \includegraphics[width=0.225\linewidth, height=0.225\linewidth]{example-image-a} & 
        \includegraphics[width=0.225\linewidth, height=0.225\linewidth]{example-image-a} \\
        % \rotatebox{90}{Text} & 
        % \includegraphics[width=0.225\linewidth, height=0.225\linewidth]{example-image-a} &
        % \includegraphics[width=0.225\linewidth, height=0.225\linewidth]{example-image-a} & 
        % \includegraphics[width=0.225\linewidth, height=0.225\linewidth]{example-image-a} & 
        % \includegraphics[width=0.225\linewidth, height=0.225\linewidth]{example-image-a} \\
        
        \bottomrule
    \end{tabular}
    \caption{T-SNE plots of embedding spaces for different pre-training methods. }
    \label{fig:my_label}
\end{figure}

==> figures/prompt_templates.tex <==
% \begin{figure*}[b]
%     \centering
%     \includegraphics[width=\linewidth]{figures/images/placeholder_templates(1).png}
%     \caption{Caption}
%     \label{fig:my_label}
% \end{figure*}

==> figures/segmentation_qual.tex <==
\begin{figure*}
    \centering
    \begin{tabular}{ccccc}
    \toprule
        Input & Supervised &  CLIP &  SLIP &  Ours \\
        \midrule
        \frame{\begin{overpic}[width=0.19\linewidth,height=0.19\linewidth]{figures/qual_samples/00003440_000.png}
        \put(3,90){\color{white}\texttt{Atelectasis}}
        \end{overpic}}&
         \includegraphics[width=0.19\linewidth,height=0.19\linewidth]{example-image-a}&
         \includegraphics[width=0.19\linewidth,height=0.19\linewidth]{example-image-a}&
         \includegraphics[width=0.19\linewidth,height=0.19\linewidth]{example-image-a}&
         \includegraphics[width=0.19\linewidth,height=0.19\linewidth]{example-image-a}\\
         \frame{\begin{overpic}[width=0.19\linewidth,height=0.19\linewidth]{figures/qual_samples/00004911_018.png}
        \put(3,90){\color{white}\texttt{Nodule}}
        \end{overpic}}&
         \includegraphics[width=0.19\linewidth,height=0.19\linewidth]{example-image-a}&
         \includegraphics[width=0.19\linewidth,height=0.19\linewidth]{example-image-a}&
         \includegraphics[width=0.19\linewidth,height=0.19\linewidth]{example-image-a}&
         \includegraphics[width=0.19\linewidth,height=0.19\linewidth]{example-image-a} \\ 
         \frame{\begin{overpic}[width=0.19\linewidth,height=0.19\linewidth]{figures/qual_samples/00018366_029.png}
        \put(3,90){\color{white}\texttt{Pneumothorax}}
        \end{overpic}}&
         \includegraphics[width=0.19\linewidth,height=0.19\linewidth]{example-image-a}&
         \includegraphics[width=0.19\linewidth,height=0.19\linewidth]{example-image-a}&
         \includegraphics[width=0.19\linewidth,height=0.19\linewidth]{example-image-a}&
         \includegraphics[width=0.19\linewidth,height=0.19\linewidth]{example-image-a} \\ 
         \bottomrule
    \end{tabular}
    
    \caption{Class Activation Mappings \cite{} of different approaches. }
    \label{fig:my_label}
\end{figure*}

==> sections/6_rebuttal.tex <==
The reviewers and I agree that moving away from a fixed set of findings in training a CAD classifier is an important and useful paradigm shift. The improvements reported are small, But I think the value is in methodology.


R1 

1. The model has four different hyper parameters \lambda_1 - \lambda_4 to weigh the contributions of various loss terms. How do they arrive at the settings mentioned below Eq. 5? Which of these parameters is the performance most sensitive to?

2. Some of the differences reported in Table 1 are rather minor and do not report a measure of standard deviation. How consistent are these differences and would they hold up under a statistical comparison?

Minor :

1. Typo in the line below Eq. 5, there are two settings for \lambda_4 mentioned

2. The explanation above Eq. 1 for breaking the symmetry is a bit hard to parse. Perhaps a few lines of explanation can be provided on which portion of the loss differs from the traditional MILNCE construction

R2


In some cases, the improvement in the results is not very big. A statistical analysis would be helpful to better understand the significance of the obtained improvement

This is a well written manuscript that presents relevant work on a widely studied topic. The reduction in the need of data annotation is a very helpful tool for any other medical image application.
A more in depth statistical analysis of the results may be helpful to better understand the impact of the improvements achieved

R3

The novelty of the framework is limited.
1. In my opinion, this work mainly adopts the existing contrastive language-image pertaining model, i.e., CLIP [1], from computer vision to a new domain or a new task. However, introducing large pre-trained models to solve a new downstream task cannot bring new insights to the community. It's very important to explain why the proposed approach can improve the performance and what problems can be solved by the approach?
2. There are some previous works, e.g., [2], that have attempted to adapt the contrastive language-image pertaining model into the medical image analysis field. The authors neither cite nor compare with it.

[1] Learning Transferable Visual Models From Natural Language Supervision. 2021.
[2] Contrastive Learning of Medical Visual Representations from Paired Images and Text. 2020.

1. The novelty of the framework is limited. In my opinion, this work mainly adopts the existing contrastive language-image pertaining model, i.e., CLIP [1], from computer vision to a new domain or a new task. However, introducing large pre-trained models to solve a new downstream task cannot bring new insights to the community. It's very important to explain why the proposed approach can improve the performance and what problems can be solved by the approach?

2. I recommend the authors add a Related Work section to help the readers better understand the differences between this work and previous works, .e.g, [2]. Besides, I recommend further discussing the advantage and disadvantage of each previous work, instead of just listing them, which can help the readers understand the strengths and weaknesses of this work.

3. Many important hyper-parameters are missing, such as learning rate, batch size, and the number of epochs, which hinder reproducibility. Besides, it is necessary to report some model details and training details for the proposed approach, for example, the training time, numbers of model parameters and memory cost, and so on.

4. The paper is written in an optimistic tone that leads the reader to assume the proposed approach is rather good. However, I am more interested in knowing if the approach brings errors? And what type of errors does it bring? And why?

5. I would like to see a statistical significance test, due to the performance gap between the proposed approach and the previous state-of-the-art methods is small.

[1] Learning Transferable Visual Models From Natural Language Supervision. 2021.
[2] Contrastive Learning of Medical Visual Representations from Paired Images and Text. 2020.

==> tables/retrieval.tex <==
\begin{table}[h]
    \centering
    \begin{tabular}{llccccccccccccccccc}
    \toprule
    & \multirow{2}{*}{Method} && \multicolumn{5}{c}{MIMIC-CXR }  && \multicolumn{5}{c}{OpenI } && \\\cline{4-8}\cline{10-14}
    & & & mAP & R1 & R5 & R10  & R50  && mAP & R1 & R5 & R10  & R50  \\ 
    \midrule 
    \multirow{6}{*}{\rotatebox{90}{I2T}} & Random                          & & 00.92 & 00.76 & 01.17 & 04.74 & 19.05 & & 00.21 & 00.03 & 00.09 & 00.19 & 00.82   \\
    & CLIP                          & & x & x & x & x & x & & x & x & x & x & x   \\
    & SLIP                        & & x & x & x & x & x & & x & x & x & x & x   \\
    & Ours                        & & - & - & - & - & - & & - & - & - & - & -   \\
    \midrule
    \multirow{6}{*}{\rotatebox{90}{T2I}} & Random                          & & 00.97 & 00.33 & 02.67 & 05.58 & 22.03 & & 00.16 & 00.03 & 00.12 & 00.30 & 01.48  \\
    & CLIP                          & & x & x & x & x & x & & x & x & x & x & x   \\
    & SLIP                        & & x & x & x & x & x & & x & x & x & x & x   \\
    & Ours                        & & - & - & - & - & - & & - & - & - & - & -   \\
    \bottomrule
    \end{tabular}
    \caption{Image-to-Text(I2T) and Text-to-Image(T2I) retrieval performance.}
    \label{tab:my_label}
\end{table}
    

==> tables/segmentation_quant.tex <==
\begin{table}[]

        \centering
        \begin{tabular}{ccccccccccccccc}
        \toprule
        \multirow{2}{*}{Init.} & \multicolumn{2}{c}{SSID (ZS)} && \multicolumn{2}{c}{SSID (1\%)} & &  \multicolumn{2}{c}{SSID (10\%)} &&  \multicolumn{2}{c}{SSID (50\%)} & & \multicolumn{2}{c}{SSID (100\%)}\\\cline{2-3}\cline{5-6}\cline{8-9}\cline{11-12}\cline{14-15}
         & mIoU & P.Acc. && mIoU & P.Acc. & & mIoU & P.Acc.& & mIoU & P.Acc.& & mIoU & P.Acc.
        \\\midrule
        
         Random             & - & - & & - & -& & - & - &&  - & - &&  - & -   \\
         ImageNet           & - & - & & - & -& & - & - &&  - & - &&  - & -   \\
         SimCLRv2           & - & - & & - & -& & - & - &&  - & - &&  - & -   \\
         CLIP               & - & - & & - & -& & - & - &&  - & - &&  - & -   \\
         RadCLIP            & - & - & & - & -& & - & - &&  - & - &&  - & -   \\
         \bottomrule
        \end{tabular}
        \caption{https://arxiv.org/pdf/2112.01071.pdf}
        \label{tab:my_label}

\end{table}
